CInC Flow: Characterizable Invertible 3x3 Convolution

Normalizing flows are an essential alternative to GANs for generative modelling, which can be optimized directly on the maximum likelihood of the dataset. They also allow computation of the exact latent vector corresponding to an image since they are composed of invertible transformations. However, the requirement of invertibility of the transformation prevents standard and expressive neural network models such as CNNs from being directly used. Emergent convolutions were proposed to construct an invertible 3$\times$3 CNN layer using a pair of masked CNN layers, making them inefficient. We study conditions such that 3$\times$3 CNNs are invertible, allowing them to construct expressive normalizing flows. We derive necessary and sufficient conditions on a padded CNN for it to be invertible. Our conditions for invertibility are simple, can easily be maintained during the training process. Since we require only a single CNN layer for every effective invertible CNN layer, our approach is more efficient than emerging convolutions. We also proposed a coupling method, Quad-coupling. We benchmark our approach and show similar performance results to emergent convolutions while improving the model's efficiency.

==> flowstep.tex <==
\tikzset{%
  >={Latex[width=2mm,length=2mm]},
  % Specifications for style of no  des:
            base/.style = {rectangle, rounded corners, draw=black,
                           % minimum width=4cm, minimum height=1cm,
                           text centered, font=\sffamily},
  activityStarts/.style = {base, fill=blue!30},
       startstop/.style = {base, fill=red!30},
    flowstep/.style = {base, fill=green!30},
         process/.style = {base, %minimum width=2.5cm, 
                           fill=orange!15, font=\ttfamily},
}

\begin{tikzpicture}[%node distance=1.5cm,
    every node/.style={font=\sffamily}, align=center]

  \node (x)							            {$x$};
  \node (actnorm)   [process,above of =x]       {Actnorm};
  
  \node (conv)  [process, above of=actnorm]    {$3\times 3$ convolution};
  
  \node (coupling)     [process, above of=conv] {Coupling layer};
  \node (out)     [above of=coupling]      {$x'$};


  \draw[->] (x) -- (actnorm);
  \draw[->] (actnorm) -- (conv);
  \draw[->] (conv) -- (coupling);
  \draw[->] (coupling) -- (out);
  
  \end{tikzpicture}


==> model.tex <==
\tikzset{%
  >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
            base/.style = {rectangle, rounded corners, draw=black,
                           %minimum width=4cm, minimum height=1cm,
                           text centered, font=\sffamily},
  activityStarts/.style = {base, fill=blue!30},
       startstop/.style = {base, fill=red!30},
    flowstep/.style = {base, fill=green!30},
         process/.style = {base, % minimum width=2.5cm, 
                            fill=orange!15, font=\ttfamily},
}


% Drawing part, node distance is 1.5 cm and every node
% is prefilled with white background
\begin{tikzpicture}[%node distance=1.5cm,
    every node/.style={font=\sffamily}, align=center]

  \node (x)							           {$x$};
  \node (squeeze)   [process,above of =x]                  {Squeeze};
  
  % Flow steps 1
  \node (fffflowstep)  [xshift=2mm,yshift=2mm,flowstep, above of=squeeze]       {\phantom{Flow Step}};
  \node (ffflowstep)  [xshift=1mm,yshift=1mm,flowstep, above of=squeeze]       {\phantom{Flow Step}};
  \node (fflowstep)  [xshift=0mm,yshift=0mm,flowstep, above of=squeeze]       {\phantom{Flow Step}};
  \draw[->] (squeeze) -- (fflowstep);
  \node (flowstep)  [xshift=-1mm,yshift=-1mm,flowstep, above of=squeeze]       {Flow Step};
  
  \node (split)     [process, above of=fflowstep, yshift=2mm]      {Split};
  \node (squeeze2)  [process, above of=split]    	  {Squeeze};
  \node (zi)        [ left = 8mm of split]					  {$z_i$};
  
  
  % Flow steps 2 
  \node (fffflowstep2)  [xshift=2mm,yshift=2mm,flowstep, above of=squeeze2]       {\phantom{Flow Step}};
  \node (ffflowstep2)  [xshift=1mm,yshift=1mm,flowstep, above of=squeeze2]       {\phantom{Flow Step}};
  \node (fflowstep2)  [xshift=0mm,yshift=0mm,flowstep, above of=squeeze2]       {\phantom{Flow Step}};
  \draw[->] (squeeze2) -- (fflowstep2);
  \node (flowstep2)  [xshift=-1mm,yshift=-1mm,flowstep, above of=squeeze2]       {Flow Step};
  
  \node (zk) [above of=fflowstep2, yshift=2mm] {$z_K$};


  % Brace flowstep 1
	\node (brace1b) [xshift=4mm, yshift=-4mm, right of = flowstep] {};
	\node (brace1t) [xshift=1mm, yshift=4mm, right of = fffflowstep] {};
	\draw [snake=brace] (brace1t) -- (brace1b) node[midway, right] {$\times D$};

  % Brace flowstep 2
	\node (brace2b) [xshift=4mm, yshift=-4mm, right of = flowstep2] {};
	\node (brace2t) [xshift=1mm, yshift=4mm, right of = fffflowstep2] {};
	\draw [snake=brace] (brace2t) -- (brace2b) node[midway, right] {$\times D$};


  \draw[->] (x) -- (squeeze);
  %\draw[->] (squeeze) -- (fflowstep);
  \draw[->] (fflowstep) -- (split);
  \draw[->] (split) -- (squeeze2);
  \draw[->] (split) -- (zi);
  %\draw[->] (squeeze2) -- (flowstep2);
  \draw[->] (fflowstep2) -- (zk);

  
  % Arrow
%  \node (timesK) [xshift=3cm, right of=fflowstep] {$\times \left(K-1\right)$};
%  \draw (split) -| (timesK);
%  \draw[->] (timesK) |-  (squeeze.east);
  
  
  % Brace
  \node (bracefb) [xshift=1.3cm, yshift=-6mm, right of = squeeze] {};
  \node (braceft) [xshift=1.3cm, yshift=6mm, right of = split] {};
  \draw [decorate,decoration={brace,amplitude=4pt}]
  (braceft) -- (bracefb) node[midway, right, xshift=0.5mm] {$\times \left(K-1\right)$};
    
\end{tikzpicture}


==> new_coupling.tex <==
\begin{tikzpicture}
\tikzstyle{dot} = [
fill,
shape=circle,
minimum size=4pt,
inner sep=0pt,
]

\tikzstyle{F} = [
thick,
trapezium, 
trapezium angle=70, 
rotate=90, 
draw,
inner ysep=5pt, 
outer sep=0pt,
minimum height=2em, 
minimum width=2em,
]

\node[opacity=0.0] (f) {};
\node[F, rotate around={0:(f.center)}] at (f) {\rotatebox{250}{$f_1$}};
\node[XOR, left = 2em of f, scale=0.8] (LeftXOR) {};
\draw[thick,-latex] ($(f)+(-1.1em,0em)$) -- (LeftXOR);

\node[dot, right = 2em of f, scale=0.8,yshift=1.5em] (B) {};
\draw[thick,-latex] (B.center) -- ($(B-|f.south)+(1.1em,0em)$);

\node[dot, right = 5em of B, scale=0.8,yshift=-1.5em] (C) {};
\draw[thick,-latex] (C.center) -- ($(C-|f.south)+(1.1em,0em)$);

\node[dot, right = 5em of C, scale=0.8,yshift=-1.5em] (D) {};
\draw[thick,-latex] (D.center) -- ($(D-|f.south)+(1.1em,0em)$);





\node[opacity=0.0, below right = 6.45em of f, yshift=1em, scale=0.8] (g) {};
\node[F, rotate around={0:(g.center)}] at (g) {\rotatebox{250}{$f_2$}};
\node[XOR, left = 2em of g, scale=0.8] (LeftXORG) {};
\draw[thick,-latex] ($(g)+(-1.1em,0em)$) -- (LeftXORG);

\node[dot, right = 2.188em of g, scale=0.8,yshift=0.75em] (BG) {};
\draw[thick,-latex] (BG.center) -- ($(BG-|g.south)+(1.1em,0em)$);

\node[dot, right = 5em of BG, scale=0.8,yshift=-1.5em] (CG) {};
\draw[thick,-latex] (CG.center) -- ($(CG-|g.south)+(1.1em,0em)$);




\node[opacity=0.0, below right = 6.73em of g,  yshift=1.5em, scale=0.8] (h) {};
\node[F, rotate around={0:(h.center)}] at (h) {\rotatebox{250}{$f_3$}};
\node[XOR, left = 2em of h, scale=0.8] (LeftXORH) {};
\draw[thick,-latex] ($(h)+(-1.1em,0em)$) -- (LeftXORH);

\node[dot, right = 2.1885em of h, scale=0.8,yshift=0em] (BH) {};
\draw[thick,-latex] (BH.center) -- ($(BH-|h.south)+(1.1em,0em)$);



\node[below = 11em of LeftXOR, draw, thick, text width=2em, align=center] (AA) {$Y_1$};
\node[draw, thick, text width=2em, align=center] (BB) at (AA-|B) {$Y_2$};
\node[draw, thick, text width=2em, align=center] (CC) at (AA-|C) {$Y_3$};
\node[draw, thick, text width=2em, align=center] (DD) at (AA-|D) {$Y_4$};


%% 4 --> 1
\draw[thick,-latex] 
(D.center) 
-- (DD);

%% 3 --> 4
\draw[thick,-latex] 
(LeftXORH) 
-- (CC);

%% 2 --> 3
\draw[thick,-latex] 
(LeftXORG) 
-- (BB);

%% 1 --> 2
\draw[thick,-latex] 
(LeftXOR.center) 
-- (AA);


%% Inputs    
\node[above = 2em of LeftXOR, draw, thick, text width=2em, align=center] (In0) {$X_1$};
\node[draw, thick, text width=2em, align=center] (In1) at (In0-|B) {$X_2$};
\node[draw, thick, text width=2em, align=center] (In2) at (In0-|C) {$X_3$};
\node[draw, thick, text width=2em, align=center] (In3) at (In0-|D) {$X_4$};

%\node[draw, thick] at (above of In1) {$X_1$};

\draw[thick,-latex] (In0) -- (LeftXOR);
\draw[thick,-latex] (In1) -- (LeftXORG);
\draw[thick,-latex] (In2) -- (LeftXORH);
\draw[thick] (In3) -- (D.center);
\end{tikzpicture}


==> tikzlibrarycrypto.symbols.code.tex <==
\usetikzlibrary{arrows}			%% Include regular arrows
\usepgflibrary{arrows.new}		%% Include custom arrows
\usetikzlibrary{shadows.blur}	%% Include the package to add shadows

%%
%% XOR in TIKZ
%%
\tikzset{XOR/.style={thick,
					draw,
					circle,
					append after command={
					        [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
					        (\tikzlastnode.north) edge[thick] (\tikzlastnode.south)
					        (\tikzlastnode.east) edge[thick] (\tikzlastnode.west)
        				},
    				},
}

%%
%% ADD in TIKZ
%%
\tikzset{ADD/.style={thick,
					draw,
					rectangle,
					append after command={
					        [shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
					        (\tikzlastnode.north) edge[thick] (\tikzlastnode.south)
					        (\tikzlastnode.east) edge[thick] (\tikzlastnode.west)
				        },
				    },
}

%%
%% MOD ADD in TIKZ
%%
\tikzset{MODADD/.style={thick,
						draw,
						rectangle,
						append after command={
								[shorten >=\pgflinewidth, shorten <=\pgflinewidth,]
								(\tikzlastnode.north) edge[thick] (\tikzlastnode.south)
								(\tikzlastnode.east) edge[thick] (\tikzlastnode.west)
							},
						},
}

%%% Shadows
\tikzset{
		%% XOR node
		shadows/.is choice,
		shadows/yes/.style={
			XOR/.append style={fill=white,blur shadow={shadow blur steps=5}},
			ADD/.append style={blur shadow={shadow blur steps=5}},
			MODADD/.append style={fill=white,blur shadow={shadow blur steps=5}}
		},
		shadows/no/.style={
		},
		%% Default: no shadows
		shadows = no,
}


%%%%%%%%%%%%%%%%%%%%%% AUTHENTICATED ENCRYPTION %%%%%%%%%%%%%%%%%%%%

%%
%% AE: Message block
%%
\tikzset{AE_msg/.style={
		rectangle,
		thick,
		draw,
		fill=blue!20,
		text width=1cm,
		minimum height=0.5cm,
		text centered,
		anchor=north,
	}
}

%%
%% AE: Ciphertext block
%%
\tikzset{AE_ctx/.style={
		rectangle,
		thick,
		draw,
		fill=green!20,
		text width=1cm, 
		minimum height=0.5cm,
		text centered,
		anchor=north,
	}
}

%%
%% AE: Tag block
%%
\tikzset{AE_tag/.style={
		rectangle,
		thick,
		draw,
		fill=red!20,
		text width=1cm, 
		minimum height=0.5cm,
		text centered,
		anchor=north,
	}
}

%%
%% AE: Block cipher call
%%
\tikzset{AE_E/.style={
		rectangle,
		thick,
		draw,
		fill=yellow!20,
		text width=1cm, 
		minimum height=1cm,
		text centered,
		anchor=north,
	}	
}

%%%%%%%%%%%%%%%%%%%%%%%%%% Custom lines or arrows %%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzset{edge/.style={
						-latex new, 
						arrow head=8pt, 
						thick
					},
}

\tikzset{line/.style={
						thick,
						draw, 
						-latex',
						shorten <=1bp,
						shorten >=1bp,
					}
}

\tikzset{doublearrow/.style={
								thick,
								draw, 
								latex-latex,
								shorten <=1bp,
								shorten >=1bp
							}
}

\tikzset{edgee/.style={
						latex new-latex new, 
						arrow head=8pt, 
						thick,
						}
}

\tikzset{Redge/.style={
						latex new-, 
						arrow head=8pt, 
						thick,
						}
}


